Weighting Scheme for a Pairwise Multi-label Classifier Based on the Fuzzy Confusion Matrix

In this work we addressed the issue of applying a stochastic classifier and a local, fuzzy confusion matrix under the framework of multi-label classification. We proposed a novel solution to the problem of correcting label pairwise ensembles. The main step of the correction procedure is to compute classifier-specific competence and cross-competence measures, which estimates error pattern of the underlying classifier. At the fusion phase we employed two weighting approaches based on information theory. The classifier weights promote base classifiers which are the most susceptible to the correction based on the fuzzy confusion matrix. During the experimental study, the proposed approach was compared against two reference methods. The comparison was made in terms of six different quality criteria. The conducted experiments reveals that the proposed approach eliminates one of main drawbacks of the original FCM-based approach i.e. the original approach is vulnerable to the imbalanced class/label distribution. What is more, the obtained results shows that the introduced method achieves satisfying classification quality under all considered quality criteria. Additionally, the impact of fluctuations of data set characteristics is reduced.

==> figures/radar.tex <==
% Created by tikzDevice version 0.10.1 on 2016-06-26 10:51:46
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,75) rectangle (480.0,460.0);
\begin{scope}
\path[clip] ( 49.20, 61.20) rectangle (480.69,456.69);
\definecolor{drawColor}{RGB}{0,0,128}
%\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 61.20) rectangle (480.69,456.69);

\path[draw=drawColor,line width= 1.5pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,289.46) --
	(238.52,274.20) --
	(238.52,243.69) --
	(264.94,228.43) --
	(291.37,243.69) --
	(291.37,274.20) --
	(264.94,289.46);
\definecolor{drawColor}{RGB}{0,0,255}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (257.32,286.02) {\Large best};
\definecolor{drawColor}{RGB}{0,0,128}

\path[draw=drawColor,line width= 1.5pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,319.98) --
	(212.09,289.46) --
	(212.09,228.43) --
	(264.94,197.91) --
	(317.80,228.43) --
	(317.80,289.46) --
	(264.94,319.98);

\path[draw=drawColor,line width= 1.5pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,350.49) --
	(185.66,304.72) --
	(185.66,213.17) --
	(264.94,167.40) --
	(344.23,213.17) --
	(344.23,304.72) --
	(264.94,350.49);

\path[draw=drawColor,line width= 1.5pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,381.01) --
	(159.23,319.98) --
	(159.23,197.91) --
	(264.94,136.88) --
	(370.66,197.91) --
	(370.66,319.98) --
	(264.94,381.01);

\path[draw=drawColor,line width= 1.5pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,411.53) --
	(132.81,335.24) --
	(132.81,182.65) --
	(264.94,106.36) --
	(397.08,182.65) --
	(397.08,335.24) --
	(264.94,411.53);
\definecolor{drawColor}{RGB}{0,0,255}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (257.32,408.45) {\Large worst};
\definecolor{drawColor}{RGB}{0,0,128}

\path[draw=drawColor,line width= 1.5pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,289.46) -- (264.94,411.53);

\path[draw=drawColor,line width= 1.5pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (238.52,274.20) -- (132.81,335.24);

\path[draw=drawColor,line width= 1.5pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (238.52,243.69) -- (132.81,182.65);

\path[draw=drawColor,line width= 1.5pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,228.43) -- (264.94,106.36);

\path[draw=drawColor,line width= 1.5pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (291.37,243.69) -- (397.08,182.65);

\path[draw=drawColor,line width= 1.5pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (291.37,274.20) -- (397.08,335.24);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (264.94,426.0) {\Large Hamming};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (110.0,348.02) {\Large Macro $F_{1}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (110.0,164.92) {\Large Micro $F_{1}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (264.94, 85.38) {\Large Ranking};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (420.51,164.92) {\Large Ex $F_{1}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (420.51,347.05) { \Large Zero-one};

\path[draw=drawColor,line width= 1.6pt,line join=round,line cap=round] (264.94,361.02) --
	(187.48,303.67) --
	(163.79,200.54) --
	(264.94,165.29) --
	(367.92,199.49) --
	(356.08,311.56) --
	(264.94,361.02);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (264.94,361.02) circle (  2.25);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (187.48,303.67) circle (  2.25);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (163.79,200.54) circle (  2.25);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (264.94,165.29) circle (  2.25);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (367.92,199.49) circle (  2.25);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (356.08,311.56) circle (  2.25);

\path[draw=drawColor,line width= 1.6pt,line join=round,line cap=round] (264.94,323.45) --
	(264.94,398.58);

\path[draw=drawColor,line width= 1.6pt,line join=round,line cap=round] (220.02,284.88) --
	(154.95,322.45);

\path[draw=drawColor,line width= 1.6pt,line join=round,line cap=round] (196.32,219.33) --
	(132.81,182.65);

\path[draw=drawColor,line width= 1.6pt,line join=round,line cap=round] (264.94,202.86) --
	(264.94,127.73);

\path[draw=drawColor,line width= 1.6pt,line join=round,line cap=round] (335.39,218.27) --
	(397.08,182.65);

\path[draw=drawColor,line width= 1.6pt,line join=round,line cap=round] (323.54,292.78) --
	(388.61,330.34);
\definecolor{drawColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 1.6pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (264.94,339.97) --
	(169.26,314.19) --
	(196.60,219.48) --
	(264.94,182.13) --
	(329.65,221.59) --
	(350.61,308.40) --
	(264.94,339.97);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (264.94,343.47) --
	(267.98,338.22) --
	(261.91,338.22) --
	(264.94,343.47);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (169.26,317.69) --
	(172.29,312.44) --
	(166.23,312.44) --
	(169.26,317.69);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (196.60,222.98) --
	(199.63,217.73) --
	(193.57,217.73) --
	(196.60,222.98);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (264.94,185.63) --
	(267.98,180.38) --
	(261.91,180.38) --
	(264.94,185.63);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (329.65,225.09) --
	(332.68,219.84) --
	(326.62,219.84) --
	(329.65,225.09);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (350.61,311.90) --
	(353.64,306.65) --
	(347.58,306.65) --
	(350.61,311.90);
\definecolor{drawColor}{RGB}{0,205,0}

\path[draw=drawColor,line width= 1.6pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,350.49) --
	(200.24,296.30) --
	(196.60,219.48) --
	(264.94,154.77) --
	(335.12,218.43) --
	(326.00,294.20) --
	(264.94,350.49);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (261.76,350.49) -- (268.13,350.49);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (264.94,347.31) -- (264.94,353.68);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (197.06,296.30) -- (203.42,296.30);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (200.24,293.12) -- (200.24,299.48);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (193.42,219.48) -- (199.78,219.48);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (196.60,216.30) -- (196.60,222.67);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (261.76,154.77) -- (268.13,154.77);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (264.94,151.59) -- (264.94,157.95);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (331.93,218.43) -- (338.30,218.43);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (335.12,215.25) -- (335.12,221.61);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (322.82,294.20) -- (329.18,294.20);

\path[draw=drawColor,line width= 1.5pt,line join=round,line cap=round] (326.00,291.01) -- (326.00,297.38);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 51.33,455.77) rectangle (130.29,381.37);%Legend frame

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 65.56,426.37) -- ( 83.56,426.37);
\definecolor{drawColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 1.2pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] ( 65.56,410.77) -- ( 83.56,410.77);
\definecolor{drawColor}{RGB}{0,205,0}

\path[draw=drawColor,line width= 1.2pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] ( 65.56,395.17) -- ( 83.56,395.17);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 74.56,426.37) circle (  2.25);
\definecolor{drawColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 74.56,414.27) --
	( 77.59,409.03) --
	( 71.53,409.03) --
	( 74.56,414.27);
\definecolor{drawColor}{RGB}{0,205,0}

\path[draw=drawColor,line width= 1.4pt,line join=round,line cap=round] ( 71.38,395.17) -- ( 77.74,395.17);

\path[draw=drawColor,line width= 1.4pt,line join=round,line cap=round] ( 74.56,391.99) -- ( 74.56,398.36);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 89.31,443.0) {\large Algorithms:  };

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 86.26,422.93) {1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 86.26,407.33) {2};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 86.26,391.73) {3};
\end{scope}
\end{tikzpicture}


==> figures/radar_J48.tex <==
% Created by tikzDevice version 0.10.1 on 2017-06-18 16:33:45
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (50,70) rectangle (480.0,460.0);
\begin{scope}
\path[clip] ( 49.20, 61.20) rectangle (480.69,456.69);
\definecolor{drawColor}{RGB}{0,0,128}

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,289.46) --
	(243.37,280.52) --
	(234.43,258.94) --
	(243.37,237.37) --
	(264.94,228.43) --
	(286.52,237.37) --
	(295.46,258.94) --
	(286.52,280.52) --
	(264.94,289.46);
\definecolor{drawColor}{RGB}{0,0,255}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (257.32,286.02) {best};
\definecolor{drawColor}{RGB}{0,0,128}

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,319.98) --
	(221.79,302.10) --
	(203.91,258.94) --
	(221.79,215.79) --
	(264.94,197.91) --
	(308.10,215.79) --
	(325.98,258.94) --
	(308.10,302.10) --
	(264.94,319.98);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,350.49) --
	(200.21,323.68) --
	(173.40,258.94) --
	(200.21,194.21) --
	(264.94,167.40) --
	(329.68,194.21) --
	(356.49,258.94) --
	(329.68,323.68) --
	(264.94,350.49);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,381.01) --
	(178.63,345.26) --
	(142.88,258.94) --
	(178.63,172.63) --
	(264.94,136.88) --
	(351.26,172.63) --
	(387.01,258.94) --
	(351.26,345.26) --
	(264.94,381.01);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,411.53) --
	(157.05,366.84) --
	(112.36,258.94) --
	(157.05,151.05) --
	(264.94,106.36) --
	(372.84,151.05) --
	(417.53,258.94) --
	(372.84,366.84) --
	(264.94,411.53);
\definecolor{drawColor}{RGB}{0,0,255}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (257.32,408.45) {worst};
\definecolor{drawColor}{RGB}{0,0,128}

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,289.46) -- (264.94,411.53);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (243.37,280.52) -- (157.05,366.84);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (234.43,258.94) -- (112.36,258.94);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (243.37,237.37) -- (157.05,151.05);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,228.43) -- (264.94,106.36);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (286.52,237.37) -- (372.84,151.05);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (295.46,258.94) -- (417.53,258.94);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (286.52,280.52) -- (372.84,366.84);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (264.94,440.0) {\Large J48};
\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (264.94,420.0) {\large Hamming};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (136.0,380.0) {\large Zero-One};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 83.85,256.47) {\large Ex $F_1$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (135.48,127.00) {\large Ranking};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (264.94, 72.40) {\large Macro $\mathrm{FDR}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (394.41,126.03) {\large Macro  $\mathrm{FNR}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (448.04,256.47) {\large Macro $F_1$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (394.41,385.94) {\large Micro $F_1$};

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (264.94,389.33) --
	(172.75,351.14) --
	(145.65,258.94) --
	(205.44,199.44) --
	(264.94,124.86) --
	(304.83,219.06) --
	(389.78,258.94) --
	(346.68,340.68) --
	(264.94,389.33);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,389.33) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (172.75,351.14) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (145.65,258.94) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (205.44,199.44) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,124.86) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (304.83,219.06) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (389.78,258.94) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (346.68,340.68) circle (  2.25);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (264.94,354.12) --
	(264.94,411.53);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (197.65,326.24) --
	(157.05,366.84);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (180.87,258.94) --
	(112.36,258.94);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (230.34,224.34) --
	(180.54,174.54);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (264.94,160.07) --
	(264.94,106.36);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (286.52,237.37) --
	(329.73,194.16);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (354.57,258.94) --
	(417.53,258.94);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (321.78,315.78) --
	(371.58,365.58);
\definecolor{drawColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 2.8pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (264.94,332.92) --
	(211.98,311.91) --
	(181.72,258.94) --
	(196.29,190.29) --
	(264.94,189.59) --
	(345.37,178.52) --
	(347.25,258.94) --
	(326.41,320.41) --
	(264.94,332.92);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,336.42) --
	(267.98,331.17) --
	(261.91,331.17) --
	(264.94,336.42);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (211.98,315.41) --
	(215.01,310.16) --
	(208.95,310.16) --
	(211.98,315.41);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (181.72,262.44) --
	(184.75,257.20) --
	(178.69,257.20) --
	(181.72,262.44);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (196.29,193.79) --
	(199.32,188.54) --
	(193.26,188.54) --
	(196.29,193.79);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,193.09) --
	(267.98,187.84) --
	(261.91,187.84) --
	(264.94,193.09);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (345.37,182.02) --
	(348.40,176.77) --
	(342.34,176.77) --
	(345.37,182.02);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (347.25,262.44) --
	(350.28,257.20) --
	(344.22,257.20) --
	(347.25,262.44);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (326.41,323.91) --
	(329.44,318.66) --
	(323.38,318.66) --
	(326.41,323.91);
\definecolor{drawColor}{RGB}{0,205,0}

\path[draw=drawColor,line width= 2.8pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,329.22) --
	(215.90,307.99) --
	(192.82,258.94) --
	(198.90,192.90) --
	(264.94,187.74) --
	(338.83,185.06) --
	(332.45,258.94) --
	(315.95,309.95) --
	(264.94,329.22);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (261.76,329.22) -- (268.13,329.22);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,326.04) -- (264.94,332.41);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (212.72,307.99) -- (219.09,307.99);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (215.90,304.80) -- (215.90,311.17);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (189.63,258.94) -- (196.00,258.94);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (192.82,255.76) -- (192.82,262.13);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (195.72,192.90) -- (202.08,192.90);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (198.90,189.72) -- (198.90,196.08);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (261.76,187.74) -- (268.13,187.74);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,184.56) -- (264.94,190.92);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (335.65,185.06) -- (342.02,185.06);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (338.83,181.87) -- (338.83,188.24);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (329.27,258.94) -- (335.63,258.94);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (332.45,255.76) -- (332.45,262.13);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (312.77,309.95) -- (319.13,309.95);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (315.95,306.77) -- (315.95,313.13);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 51.33,455.77) rectangle (107.29,381.37);

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 65.56,426.37) -- ( 83.56,426.37);
\definecolor{drawColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 0.7pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] ( 65.56,410.77) -- ( 83.56,410.77);
\definecolor{drawColor}{RGB}{0,205,0}

\path[draw=drawColor,line width= 0.7pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] ( 65.56,395.17) -- ( 83.56,395.17);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 74.56,426.37) circle (  2.25);
\definecolor{drawColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 74.56,414.27) --
	( 77.59,409.03) --
	( 71.53,409.03) --
	( 74.56,414.27);
\definecolor{drawColor}{RGB}{0,205,0}

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 71.38,395.17) -- ( 77.74,395.17);

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 74.56,391.99) -- ( 74.56,398.36);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 79.31,443.77) {Algorithms:     };

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 86.26,422.93) {1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 86.26,407.33) {2};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 86.26,391.73) {3};
\end{scope}
\end{tikzpicture}


==> figures/radar_NB.tex <==
% Created by tikzDevice version 0.10.1 on 2017-06-18 16:34:02
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (50,70) rectangle (480.0,460.0);
\begin{scope}
\path[clip] ( 49.20, 61.20) rectangle (480.69,456.69);
\definecolor{drawColor}{RGB}{0,0,128}

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,289.46) --
	(243.37,280.52) --
	(234.43,258.94) --
	(243.37,237.37) --
	(264.94,228.43) --
	(286.52,237.37) --
	(295.46,258.94) --
	(286.52,280.52) --
	(264.94,289.46);
\definecolor{drawColor}{RGB}{0,0,255}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (257.32,286.02) {best};
\definecolor{drawColor}{RGB}{0,0,128}

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,319.98) --
	(221.79,302.10) --
	(203.91,258.94) --
	(221.79,215.79) --
	(264.94,197.91) --
	(308.10,215.79) --
	(325.98,258.94) --
	(308.10,302.10) --
	(264.94,319.98);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,350.49) --
	(200.21,323.68) --
	(173.40,258.94) --
	(200.21,194.21) --
	(264.94,167.40) --
	(329.68,194.21) --
	(356.49,258.94) --
	(329.68,323.68) --
	(264.94,350.49);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,381.01) --
	(178.63,345.26) --
	(142.88,258.94) --
	(178.63,172.63) --
	(264.94,136.88) --
	(351.26,172.63) --
	(387.01,258.94) --
	(351.26,345.26) --
	(264.94,381.01);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,411.53) --
	(157.05,366.84) --
	(112.36,258.94) --
	(157.05,151.05) --
	(264.94,106.36) --
	(372.84,151.05) --
	(417.53,258.94) --
	(372.84,366.84) --
	(264.94,411.53);
\definecolor{drawColor}{RGB}{0,0,255}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (257.32,408.45) {worst};
\definecolor{drawColor}{RGB}{0,0,128}

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,289.46) -- (264.94,411.53);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (243.37,280.52) -- (157.05,366.84);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (234.43,258.94) -- (112.36,258.94);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (243.37,237.37) -- (157.05,151.05);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,228.43) -- (264.94,106.36);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (286.52,237.37) -- (372.84,151.05);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (295.46,258.94) -- (417.53,258.94);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (286.52,280.52) -- (372.84,366.84);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (264.94,440.0) {\Large Na\"{i}ve Bayes};
\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (264.94,420.0) {\large Hamming};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (136.0,380.0) {\large Zero-One};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 83.85,256.47) {\large Ex $F_1$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (135.48,127.00) {\large Ranking};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (264.94, 72.40) {\large Macro $\mathrm{FDR}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (394.41,126.03) {\large Macro  $\mathrm{FNR}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (448.04,256.47) {\large Macro $F_1$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (394.41,385.94) {\large Micro $F_1$};

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (264.94,393.03) --
	(172.75,351.14) --
	(143.80,258.94) --
	(206.75,200.75) --
	(264.94,134.11) --
	(299.60,224.29) --
	(384.24,258.94) --
	(347.99,341.99) --
	(264.94,393.03);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,393.03) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (172.75,351.14) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (143.80,258.94) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (206.75,200.75) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,134.11) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (299.60,224.29) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (384.24,258.94) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (347.99,341.99) circle (  2.25);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (264.94,357.82) --
	(264.94,411.53);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (197.65,326.24) --
	(157.05,366.84);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (179.02,258.94) --
	(112.36,258.94);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (231.65,225.65) --
	(181.85,175.85);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (264.94,169.32) --
	(264.94,106.36);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (286.52,237.37) --
	(324.50,199.39);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (349.02,258.94) --
	(417.53,258.94);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (323.09,317.09) --
	(372.84,366.84);
\definecolor{drawColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 2.8pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (264.94,332.00) --
	(208.06,315.83) --
	(179.87,258.94) --
	(195.63,189.63) --
	(264.94,178.49) --
	(347.33,176.56) --
	(349.10,258.94) --
	(325.76,319.76) --
	(264.94,332.00);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,335.50) --
	(267.98,330.25) --
	(261.91,330.25) --
	(264.94,335.50);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (208.06,319.33) --
	(211.09,314.08) --
	(205.03,314.08) --
	(208.06,319.33);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (179.87,262.44) --
	(182.90,257.20) --
	(176.84,257.20) --
	(179.87,262.44);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (195.63,193.13) --
	(198.66,187.88) --
	(192.60,187.88) --
	(195.63,193.13);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,181.99) --
	(267.98,176.74) --
	(261.91,176.74) --
	(264.94,181.99);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (347.33,180.05) --
	(350.36,174.81) --
	(344.30,174.81) --
	(347.33,180.05);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (349.10,262.44) --
	(352.13,257.20) --
	(346.07,257.20) --
	(349.10,262.44);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (325.76,323.26) --
	(328.79,318.01) --
	(322.73,318.01) --
	(325.76,323.26);
\definecolor{drawColor}{RGB}{0,205,0}

\path[draw=drawColor,line width= 2.8pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,326.45) --
	(219.83,304.06) --
	(196.51,258.94) --
	(198.25,192.25) --
	(264.94,189.59) --
	(342.10,181.79) --
	(336.15,258.94) --
	(315.29,309.29) --
	(264.94,326.45);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (261.76,326.45) -- (268.13,326.45);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,323.27) -- (264.94,329.63);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (216.64,304.06) -- (223.01,304.06);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (219.83,300.88) -- (219.83,307.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (193.33,258.94) -- (199.70,258.94);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (196.51,255.76) -- (196.51,262.13);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (195.07,192.25) -- (201.43,192.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (198.25,189.07) -- (198.25,195.43);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (261.76,189.59) -- (268.13,189.59);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,186.41) -- (264.94,192.77);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (338.92,181.79) -- (345.29,181.79);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (342.10,178.60) -- (342.10,184.97);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (332.97,258.94) -- (339.33,258.94);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (336.15,255.76) -- (336.15,262.13);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (312.11,309.29) -- (318.48,309.29);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (315.29,306.11) -- (315.29,312.48);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 51.33,455.77) rectangle (107.29,381.37);

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 65.56,426.37) -- ( 83.56,426.37);
\definecolor{drawColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 0.7pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] ( 65.56,410.77) -- ( 83.56,410.77);
\definecolor{drawColor}{RGB}{0,205,0}

\path[draw=drawColor,line width= 0.7pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] ( 65.56,395.17) -- ( 83.56,395.17);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 74.56,426.37) circle (  2.25);
\definecolor{drawColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 74.56,414.27) --
	( 77.59,409.03) --
	( 71.53,409.03) --
	( 74.56,414.27);
\definecolor{drawColor}{RGB}{0,205,0}

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 71.38,395.17) -- ( 77.74,395.17);

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 74.56,391.99) -- ( 74.56,398.36);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 79.31,443.77) {Algorithms:     };

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 86.26,422.93) {1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 86.26,407.33) {2};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 86.26,391.73) {3};
\end{scope}
\end{tikzpicture}


==> figures/radar_VPe.tex <==
% Created by tikzDevice version 0.10.1 on 2017-06-18 16:34:06
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (50,70) rectangle (480.0,460.0);
\begin{scope}
\path[clip] ( 49.20, 61.20) rectangle (480.69,456.69);
\definecolor{drawColor}{RGB}{0,0,128}

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,289.46) --
	(243.37,280.52) --
	(234.43,258.94) --
	(243.37,237.37) --
	(264.94,228.43) --
	(286.52,237.37) --
	(295.46,258.94) --
	(286.52,280.52) --
	(264.94,289.46);
\definecolor{drawColor}{RGB}{0,0,255}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (257.32,286.02) {best};
\definecolor{drawColor}{RGB}{0,0,128}

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,319.98) --
	(221.79,302.10) --
	(203.91,258.94) --
	(221.79,215.79) --
	(264.94,197.91) --
	(308.10,215.79) --
	(325.98,258.94) --
	(308.10,302.10) --
	(264.94,319.98);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,350.49) --
	(200.21,323.68) --
	(173.40,258.94) --
	(200.21,194.21) --
	(264.94,167.40) --
	(329.68,194.21) --
	(356.49,258.94) --
	(329.68,323.68) --
	(264.94,350.49);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,381.01) --
	(178.63,345.26) --
	(142.88,258.94) --
	(178.63,172.63) --
	(264.94,136.88) --
	(351.26,172.63) --
	(387.01,258.94) --
	(351.26,345.26) --
	(264.94,381.01);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,411.53) --
	(157.05,366.84) --
	(112.36,258.94) --
	(157.05,151.05) --
	(264.94,106.36) --
	(372.84,151.05) --
	(417.53,258.94) --
	(372.84,366.84) --
	(264.94,411.53);
\definecolor{drawColor}{RGB}{0,0,255}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (257.32,408.45) {worst};
\definecolor{drawColor}{RGB}{0,0,128}

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,289.46) -- (264.94,411.53);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (243.37,280.52) -- (157.05,366.84);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (234.43,258.94) -- (112.36,258.94);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (243.37,237.37) -- (157.05,151.05);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,228.43) -- (264.94,106.36);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (286.52,237.37) -- (372.84,151.05);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (295.46,258.94) -- (417.53,258.94);

\path[draw=drawColor,line width= 2.1pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (286.52,280.52) -- (372.84,366.84);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (264.94,440.0) {\Large Voted Perceptron};
\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (264.94,420.0) {\large Hamming};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (136.0,380.0) {\large Zero-One};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 83.85,256.47) {\large Ex $F_1$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (135.48,127.00) {\large Ranking};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (264.94, 72.40) {\large Macro $\mathrm{FDR}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (394.41,126.03) {\large Macro  $\mathrm{FNR}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (448.04,256.47) {\large Macro $F_1$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (394.41,385.94) {\large Micro $F_1$};
\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (264.94,393.03) --
	(173.40,350.49) --
	(143.80,258.94) --
	(210.67,204.67) --
	(264.94,124.86) --
	(302.22,221.67) --
	(389.78,258.94) --
	(350.60,344.60) --
	(264.94,393.03);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,393.03) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (173.40,350.49) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (143.80,258.94) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (210.67,204.67) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,124.86) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (302.22,221.67) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (389.78,258.94) circle (  2.25);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (350.60,344.60) circle (  2.25);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (264.94,357.82) --
	(264.94,411.53);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (198.30,325.59) --
	(157.05,366.84);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (179.02,258.94) --
	(112.36,258.94);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (235.57,229.57) --
	(185.77,179.77);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (264.94,160.07) --
	(264.94,106.36);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (286.52,237.37) --
	(327.12,196.77);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (354.57,258.94) --
	(417.53,258.94);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (325.70,319.70) --
	(372.84,366.84);
\definecolor{drawColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 2.8pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (264.94,331.07) --
	(210.67,313.22) --
	(187.27,258.94) --
	(195.63,189.63) --
	(264.94,184.97) --
	(340.80,183.09) --
	(342.62,258.94) --
	(319.87,313.87) --
	(264.94,331.07);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,334.57) --
	(267.98,329.32) --
	(261.91,329.32) --
	(264.94,334.57);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (210.67,316.72) --
	(213.70,311.47) --
	(207.64,311.47) --
	(210.67,316.72);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (187.27,262.44) --
	(190.30,257.20) --
	(184.24,257.20) --
	(187.27,262.44);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (195.63,193.13) --
	(198.66,187.88) --
	(192.60,187.88) --
	(195.63,193.13);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,188.47) --
	(267.98,183.22) --
	(261.91,183.22) --
	(264.94,188.47);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (340.80,186.59) --
	(343.83,181.34) --
	(337.77,181.34) --
	(340.80,186.59);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (342.62,262.44) --
	(345.65,257.20) --
	(339.59,257.20) --
	(342.62,262.44);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (319.87,317.37) --
	(322.90,312.12) --
	(316.84,312.12) --
	(319.87,317.37);
\definecolor{drawColor}{RGB}{0,205,0}

\path[draw=drawColor,line width= 2.8pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (264.94,327.38) --
	(216.56,307.33) --
	(189.12,258.94) --
	(194.33,188.33) --
	(264.94,192.36) --
	(346.03,177.86) --
	(337.07,258.94) --
	(318.56,312.56) --
	(264.94,327.38);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (261.76,327.38) -- (268.13,327.38);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,324.19) -- (264.94,330.56);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (213.38,307.33) -- (219.74,307.33);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (216.56,304.15) -- (216.56,310.51);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (185.93,258.94) -- (192.30,258.94);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (189.12,255.76) -- (189.12,262.13);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (191.14,188.33) -- (197.51,188.33);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (194.33,185.14) -- (194.33,191.51);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (261.76,192.36) -- (268.13,192.36);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (264.94,189.18) -- (264.94,195.55);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (342.84,177.86) -- (349.21,177.86);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (346.03,174.68) -- (346.03,181.05);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (333.89,258.94) -- (340.26,258.94);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (337.07,255.76) -- (337.07,262.13);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (315.38,312.56) -- (321.75,312.56);

\path[draw=drawColor,line width= 2.1pt,line join=round,line cap=round] (318.56,309.38) -- (318.56,315.75);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 51.33,455.77) rectangle (107.29,381.37);

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 65.56,426.37) -- ( 83.56,426.37);
\definecolor{drawColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 0.7pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] ( 65.56,410.77) -- ( 83.56,410.77);
\definecolor{drawColor}{RGB}{0,205,0}

\path[draw=drawColor,line width= 0.7pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] ( 65.56,395.17) -- ( 83.56,395.17);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 74.56,426.37) circle (  2.25);
\definecolor{drawColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 74.56,414.27) --
	( 77.59,409.03) --
	( 71.53,409.03) --
	( 74.56,414.27);
\definecolor{drawColor}{RGB}{0,205,0}

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 71.38,395.17) -- ( 77.74,395.17);

\path[draw=drawColor,line width= 0.7pt,line join=round,line cap=round] ( 74.56,391.99) -- ( 74.56,398.36);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 79.31,443.77) {Algorithms:     };

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 86.26,422.93) {1};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 86.26,407.33) {2};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 86.26,391.73) {3};
\end{scope}
\end{tikzpicture}

